A Communication- and Memory-Aware Model for Load Balancing Tasks

While load balancing in distributed-memory computing has been well-studied, we present an innovative approach to this problem: a unified, reduced-order model that combines three key components to describe "work" in a distributed system: computation, communication, and memory. Our model enables an optimizer to explore complex tradeoffs in task placement, such as increased parallelism at the expense of data replication, which increases memory usage. We propose a fully distributed, heuristic-based load balancing optimization algorithm, and demonstrate that it quickly finds close-to-optimal solutions. We formalize the complex optimization problem as a mixed-integer linear program, and compare it to our strategy. Finally, we show that when applied to an electromagnetics code, our approach obtains up to 2.3x speedups for the imbalanced execution.

==> Makefile <==
DOC_NAME=paper

all: $(DOC_NAME).pdf $(FIG_FILES)

TEX_FILES=\
	abstract.tex \
	10.tex \
        20.tex \
	30.tex \
	40.tex \
	50.tex \
	70.tex \
	80.tex \
	90.tex \
	100.tex \
	ccm-lb-segment-1.tex

$(DOC_NAME).pdf: $(DOC_NAME).tex $(TEX_FILES) $(FIG_FILES)
	latexmk -pdflatex="pdflatex -interactive=nonstopmode" -use-make $<

clean:
	rm -f $(DOC_NAME).pdf *~ *.bbl *.blg *.toc *.ilg \
	*.ind *.idx *.lof *.log *.lot *.aux *.out *.tpt
	latexmk -C


